Marinarium: A Modular Experimental Facility for Reproducible Maritime and Space-Analog Field Robotics

Field robotics research in maritime and space domains is constrained by a persistent gap between low-cost, low-fidelity simulation and costly offshore experimentation. Instrumented water tanks partially bridge this gap but often provide limited sensing, restricted experimental capabilities, and weak integration with simulation tools. To address these limitations, we present Marinarium, a modular, standalone experimental facility that provides a cost-effective intermediate testbed between simulation and field deployment. Marinarium combines a fully instrumented underwater and aerial operational volume with motion capture (MoCap), a retractable roof enabling both sheltered and open-air operation, a digital twin implemented in SMaRCSim, and direct integration with a planar space robotics laboratory, enabling both maritime and underwater space-analog experimentation. We present the design rationale of the facility and validate its capabilities through four representative studies in field robotics: (i) data-driven system identification of underwater vehicle dynamics; (ii) heterogeneous multi-domain robotic rendezvous; (iii) sim-to-real transfer for underwater robotics using learned dynamics residuals; and (iv) cross-domain validation of spacecraft autonomy using underwater surrogates. Together, these studies demonstrate that Marinarium enables reproducible, instrumented experimentation across multiple field robotics challenges that would otherwise require costly offshore deployments or be impractical to investigate using simulation alone.

==> glossary.tex <==
%------------------------------------------------------------------------------%
% List of all acronyms used somewhere
%------------------------------------------------------------------------------%

%-----A-----%
\newacronym{adcp}{ADCP}{Acoustic Doppler Current Profiler}
\newacronym{agv}{AGV}{Autonomous Ground Vehicle}
\newacronym{ahrs}{AHRS}{Attitude and Heading Reference System}
\newacronym{ai}{AI}{Artificial Intelligence}
\newacronym{aoa}{AoA}{Angle of Attack}
\newacronym{aop}{AOP}{Apparent Optical Property}
\newacronym{auv}{AUV}{Autonomous Underwater Vehicle}
\newacronym{ar}{AR}{Augmented Reality}
\newacronym{asta}{ASTA}{Autonomous Systems Test Arena}
\newacronym{atmos}{ATMOS}{Autonomy Testbed for Multi-purpose Orbiting Systems}
\newacronym{aw}{AW}{above-water}

%-----B-----%
\newacronym{bdi}{BDI}{Beliefs Desires Intentions}
\newacronym{bo}{BO}{Bayesian Optimization}
\newacronym{bt}{BT}{Behavioural Tree}
%-----C-----%
\newacronym{cad}{CAD}{Computer Aided Design}
\newacronym{can}{CAN}{Controller Area Network}
\newacronym{cb}{CB}{Center of Buoyancy}
\newacronym{cbf}{CBF}{Control Barrier Function}
\newacronym{cf}{CF}{Center of flotation}
\newacronym{cfd}{CFD}{Computational Fluid Dynamics}
\newacronym{cg}{CG}{Center of Gravity}
\newacronym{cnn}{CNN}{Convolutional Neural Network}
\newacronym{co}{CO}{Coordinate origin}
\newacronym{cog}{CoG}{Center of Gravity}
\newacronym{cps}{CPS}{Cyber-Physical System}
\newacronym{cr}{CR}{Center of Rotation}
\newacronym{ctd}{CTD}{Conudctivity, Temperature, Depth}

%-----D-----%
\newacronym{di}{DI}{Double Integrator-like}
\newacronym{dig}{DIG}{Dynamic Interaction Graph}
\newacronym{dnf}{DNF}{Decentralized Navigation Function}
\newacronym{dof}{DoF}{Degree of Freedom}
\newacronym{dol}{DOL}{Digital Ocean Lab}
\newacronym{dqn}{DQN}{Deep Q-Learning Network}
\newacronym{dr}{DR}{Dead Reckoning}
\newacronym{drl}{DRL}{Deep Reinforcement Learning}
\newacronym{dt}{DT}{digital twin}
\newacronym{dtu}{DTU}{Technical University of Danmark}
\newacronym{dvl}{DVL}{Doppler Velocity Log}

%-----E-----%
\newacronym{ecef}{ECEF}{Earth-centered Earth-fixed (frame)}
\newacronym{eci}{ECI}{Earth-centered inertial (frame)}
\newacronym{edmdc}{EDMDc}{Extended Dynamic Mode Decomposition with control}
\newacronym{ekf}{EKF}{Extended Kalman Filter}
\newacronym{enu}{ENU}{East-North-Up}
\newacronym{erm}{ERM}{Empirical Risk Minimization}
\newacronym{esa}{ESA}{the European Space Agency}

%-----F-----%
%-----G-----%
\newacronym{gis}{GIS}{Geographical Information System}
\newacronym[firstplural=Gaussian Processes]{gp}{GP}{Gaussian Process}
\newacronym{gpr}{GPR}{Gaussian Process Regression}
\newacronym{gps}{GPS}{Global Positioning System}
\newacronym{gpu}{GPU}{Graphical Processing Unit}
\newacronym{grv}{GRV}{Gaussian Random Variable}

%-----H-----%
\newacronym{hil}{HIL}{Hardware-in-the-Loop}
%-----I-----%
\newacronym{ibvs}{IBVS}{Image-Based Visual Servoing}
\newacronym{imu}{IMU}{Inertia Measurement Unit}
\newacronym{ins}{INS}{Inertial Navigation System}
\newacronym{iop}{IOP}{Inherent Optical Property}
\newacronym{iss}{ISS}{Input-to-State Stability}
\newacronym{isss}{ISSS}{Interferometric Side Scan Sonar}
\newacronym{ivp}{IVP}{Interval of Valid Prediction}
%-----J-----%
\newacronym{jsc}{JSC}{Johnson Space Center}
%-----K-----%
\newacronym{kth}{KTH}{KTH Royal Institute of Technology}

%-----L-----%
\newacronym{lars}{LARS}{Launch and Recovery System}
\newacronym{lbl}{LBL}{Long Baseline}
\newacronym{lcf}{LCF}{Longitudinal Center of Flotation}
\newacronym{lcg}{LCG}{Longitudinal Center of Gravity}
\newacronym{lm}{LM}{Levenberg-Marquardt}
\newacronym{lqg}{LQG}{Linear Quadratic Gaussian}
\newacronym{lqr}{LQR}{Linear Quadratic Regulator}
\newacronym{lti}{LTI}{Linear Time Invariant}
\newacronym{lut}{LUT}{Look-Up Table}
\newacronym{lvs}{LVS}{Laser Vision System}

%-----M-----%
\newacronym{mbes}{MBES}{Multi-Beam Echo Sounder}
\newacronym{mcts}{MCTS}{Monte Carlo Tree Search}
\newacronym{mdp}{MDP}{Markov Decision Process}
\newacronym{mimo}{MIMO}{Multi-input Multi-output}
\newacronym{ml}{ML}{Machine Learning}
\newacronym{mlp}{MLP}{Multilayer Perceptron}
% \newacronym{mocap}{MoCap}{Motion Capture}
\newacronym[shortplural={MoCaps}, longplural={Motion-Capture Systems}]{mocap}{MoCap}{Motion-Capture System}
\newacronym{mpc}{MPC}{Model Predictive Control}
\newacronym{mse}{MSE}{Mean Squared Error}

%-----N-----%
\newacronym{naf}{NAF}{Normalized Advantage Functions}
\newacronym{ned}{NED}{North-East-Down}
\newacronym{nfq}{NFQ}{Neural Fitted Q Iteration}
\newacronym{nm}{NM}{Network Manager}
\newacronym{nmpc}{N-MPC}{Non-linear Model Predictive Control}
\newacronym{nn}{NN}{Neural Network}
\newacronym{nse}{NSE}{Navier-Stokes Equation}

%-----O-----%
\newacronym{ocp}{OCP}{Optimal Control Problem}
\newacronym{ode}{ODE}{Ordinary Differential Equation}
%-----P-----%
\newacronym{pac}{PAC}{Probably Approximately Correct}
\newacronym{pbvs}{PBVS}{Position-Based Visual Servoing}
\newacronym{pd}{PD}{Proportional-Derivative}
\newacronym{pi}{PI}{Proportional-Integral}
\newacronym{pid}{PID}{Proportional-Integral-Derivative}
\newacronym{pilco}{PILCO}{Probabilistic Inference for Learning Control}
\newacronym{piml}{PIML}{Physics-informed Machine Learning}
\newacronym{pinc}{PINc}{Physics-informed Neural network with control}
\newacronym{pnp}{PnP}{Perspective-n-Point}
\newacronym{proxop}{ProxOp}{Proximity Operation}
\newacronym{pwm}{PWM}{Pulse-Width Modulation}
%-----Q-----%
%-----R-----%
\newacronym{ransac}{RANSAC}{Random Sample Consensus}
\newacronym{rbf}{RBF}{Radial Basis Function}
\newacronym{rgb}{RGB}{RGB cameras}
\newacronym{rl}{RL}{Reinforcement Learning}
\newacronym{roi}{ROI}{Region of Interest}
\newacronym{rmse}{RMSE}{Root Mean Square Error}
\newacronym{ros}{ROS}{Robot Operating System}
\newacronym{rov}{ROV}{Remotely Operated Vehicle}
\newacronym{rpm}{RPM}{Revolutions Per Minute}
\newacronym{rrm}{RRM}{Regularized Risk Minimization}
\newacronym{rk4}{RK4}{Runge-Kutta 4}
\newacronym{rrt}{RRT}{Rapidly Exploring Random Tree}
\newacronym{rsme}{RSME}{Root-Square Mean Error}
\newacronym{rss}{RSS}{Relative State Specification}

%-----S-----%
\newacronym{sam}{SAM}{Small and Affordable Maritime Robot}
\newacronym{sbl}{SBL}{Short Baseline}
\newacronym{sbp}{SBP}{Sub-bottom Profiler}
\newacronym{sdg}{SDG}{Sustainable Development Goal}
\newacronym{sgd}{SGD}{Stochastic Gradient Descent}
\newacronym{sig}{SIG}{Static Interaction Graph}
\newacronym{sil}{SIL}{Software-in-the-loop}
\newacronym{sindy}{SINDY}{Sparse Identification of Nonlinear Dynamics}
\newacronym{slam}{SLAM}{Simultaneous Localization and Mapping}
\newacronym{smarc}{SMaRC}{the Swedish Maritime Robotics Center}
\newacronym{sofar}{SOFAR}{Sound Fixing And Ranging}
\newacronym{svm}{SVM}{Support Vector Machine}
\newacronym{sysid}{SYSID}{System Identification}

%-----T-----%
\newacronym{tcg}{TCG}{Transversal Center of Gravity}
\newacronym{tcp}{TCP}{Tool Center Point}
\newacronym{td}{TD}{Temporal Difference}
\newacronym{tms}{TMS}{Tether Management System}
\newacronym{tvg}{TVG}{Time Varied Gain}


%-----U-----%
\newacronym{uav}{UAV}{Unmanned Aerial Vehicle}
\newacronym{ude}{UDE}{Universal Differential Equation}
\newacronym{usbl}{USBL}{Ultra-Short Baseline}
\newacronym{usc}{USC}{Underwater Sound Channel}
\newacronym{usv}{USV}{Unmanned Surface Vehicle}
\newacronym{uuv}{UUV}{Unmanned Underwater Vehicle}
\newacronym{uv}{UV}{Ultraviolet}
\newacronym{uw}{UW}{underwater}
\newacronym{uwb}{UWB}{Ultra-Wideband localization}
%-----V-----%
\newacronym{vbs}{VBS}{Variable Buoyancy System}
\newacronym{vc}{VC}{Vapnik-Chervonenkis}
\newacronym{vr}{VR}{Virtual Reality}
\newacronym{vta}{VTA}{Visual Tracking Algorithm}
%-----W-----%
%-----X-----%
%-----Y-----%
%-----Z-----%

